D-Box: DMA-enabled Compartmentalization for Embedded Applications

Embedded and Internet-of-Things (IoT) devices have seen an increase in adoption in many domains. The security of these devices is of great importance as they are often used to control critical infrastructure, medical devices, and vehicles. Existing solutions to isolate microcontroller (MCU) resources in order to increase their security face significant challenges such as specific hardware unavailability, Memory Protection Unit (MPU) limitations and a significant lack of Direct Memory Access (DMA) support. Nevertheless, DMA is fundamental for the power and performance requirements of embedded applications. In this paper, we present D-Box, a systematic approach to enable secure DMA operations for compartmentalization solutions of embedded applications using real-time operating systems (RTOS). D-Box defines a reference architecture and a workflow to protect DMA operations holistically. It provides practical methods to harden the kernel and define capability-based security policies for easy definition of DMA operations with strong security properties. We implemented a D-Box prototype for the Cortex-M3/M4 on top of the popular FreeRTOS-MPU (F-MPU). The D-Box procedures and a stricter security model enabled DMA operations, yet it exposed 41 times less ROP (return-orienting-programming) gadgets when compared with the standard F-MPU. D-Box adds only a 2% processor overhead while reducing the power consumption of peripheral operation benchmarks by 18.2%. The security properties and performance of D-Box were tested and confirmed on a real-world case study of a Programmable Logic Controller (PLC) application.

==> Makefile <==
# Set this to one or more main LaTeX files (e.g. those with \documentclass) 
# for a specific build. Leave blank to build all files having an uncommented
# \documentclass.
MAIN=main.tex	


###########################################################################
#                 MAKE NO EDITS BELOW (except to debug)                   #
###########################################################################
#
#
# This is the PDFLATEX makefile, no support for ps/eps/dvi.
#
# Originally based on 
#   http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/Makefile
# but redeveloped by JG. Reuse by changing just the first line to list
# the main LaTeX source file.
#
# Features:
# - Finds all included LaTeX files, including includes within includes.
# - Finds all bibs and PDF figures included.
# - Automatically generates dependency information.
# - Repeats calls to PDFLATEX as necessary to fix cross references.
# - Displays missing references in a clean format at the end of the build.
# - Finds main LaTeX source files, so this makefile is reusable wihtout edits.
# - Works for files with bibliographies, and files without.

ifndef MAIN
MAIN:=	$(shell egrep -l "documentclass" *.tex)	
endif

ALLTEX:=$(shell ls *.tex)
ALLPDF:=$(ALLTEX:.tex=.pdf)

all pdf: $(MAIN:.tex=.pdf)
help ps dvi $(MAIN:.tex=.ps) $(MAIN:.tex=.dvi): die_unsupported
$(filter-out $(MAIN:.tex=.pdf),$(ALLPDF)): die_unsupported

%.pdf: %.fig
	rm -f $@
	fig2dev -L pdf $< > $@

%.aux: %.tex
	$(LATEX) $<

%.bbl: %.tex
	bibtex $(<:.tex=)
	$(LATEX) $<

%.pdf: %.aux
	@while (grep -q "Rerun to get" $(<:.aux=.log)) do \
		$(LATEX) $(<:.aux=.tex); \
	done
	@egrep -i "(Reference|Citation).*undefined" $(<:.aux=.log) ; true
	$(LATEX) $(<:.aux=.tex)

%.dep: %.tex
	@$(gettexs); $(getbibs); $(getfigs); \
	echo "$(<:.tex=.dep): Makefile " $$texs $$bibs $$figs > $@; \
	echo "$(<:.tex=.aux): " $$texs $$figs >> $@; \
	if [ $${#bibs} -gt 0 ]; then \
		echo "$(<:.tex=.bbl): " $$texs $$bibs >> $@; \
		echo "$(<:.tex=.pdf): $(<:.tex=.bbl)" >> $@; \
	fi

vpath %.fig figs

-include $(MAIN:.tex=.dep)

.PHONY: clean die_unsupported

double:
	for i in $(ALLTEX); do echo "Double words in $$i:" && ./double.pl < $$i; done

clean:
	rm -f *~ *.log *.aux *.dvi *.bbl *.blg *.cb *.dep *.pdf *.fls *.out *.gz $(TARGET)

die_unsupported:
	$(warning Unsupported Makefile build target. Supported targets are:)
	$(warning  <BLANK> all pdf $(TARGET) clean)
	$(error Exiting)

LATEX=	pdflatex #--interaction batchmode
TARGET=	$(MAIN:.tex=.pdf)

# 9 Dec 2008 JG: This is now a worklist algorithm to pick up all recursive
#   child dependencies of discovered includes.
define gettexs
  worklist="$< "; \
  while [ $${#worklist} -gt 0 ]; do \
    curr=$${worklist%% *}; \
    worklist=$${worklist#* }; \
    texs="$${texs}$$curr "; \
    worklist=$${worklist}`perl -ne '\
               ($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/; \
	       @_=split /,/; \
	       foreach $$t (@_) { \
	         if ($$t !~ /\.tex$$/) { $$t .= ".tex"; } \
                 if (-e $$t) { print "$$t " } \
	       }' $${curr}`; \
	done
endef

define getbibs
  bibs=`perl -ne '\
        ($$_)=/^[^%]*\\\bibliography\{(.*?)\}/; \
        @_=split /,/; \
        foreach $$b (@_) { \
          if (-e "$$b.bib") { print "$$b.bib " } \
        }' $$texs`
endef

define getfigs
  figs=`perl -ne '\
        ($$_)=/^[^%]*\\\includegraphics(?:\[.*?\])?\{(.*?)\}/g; \
        if (defined($$_)) { \
          if ($$_ !~ /\.pdf$$/) { $$_ .= ".pdf"; } \
          if (-e $$_) { print "$$_ "; } \
        }' $$texs`
endef


==> overview.tex <==
\section{Overview}

==> survey.tex <==
\section{Survey on availability of hardware security features on MCUs}
\label{sec:survey}

The main isolation components of the Cortex-M embedded architecture
are the MPU and TrustZone. These two
components are optional, and their support depends on the MCU vendor
implementation. Also, each component is only supported by specific
Cortex-M micro-architecture profiles. The MPU is supported by Armv6-M
(Cortex-M0+), Armv7-M (Cortex-M3/M4/M7) and Armv8-M
(Cortex-M23/M33/M55), whereas TrustZone is exclusively supported by
the Armv8-M (Cortex-M23/M33/M55).


To verify the current availability of the ARM TrustZone feature in
commercial MCU devices, we surveyed the complete portfolio of the top
five global MCU vendors. The results depicted in Figure
\ref{fig:TZavailablity} demonstrates that TrustZone-enabled devices
are still scarce. In the best case, ST Microelectronics commercializes
16 parts which represents only 1.6\% of its portfolio. In contrast,
Cypress/Infineon has no Armv8-M commercial devices at all. Also, no
vendor currently offers commercial devices for the Cortex-M55
micro-architecture. Note that this offer is slightly better compared
to the total absence of devices supporting this technology around
2017-2018 as observed by \cite{clementsACESAutomaticCompartments2018}.


\begin{figure}
    \centering
    \includegraphics[width=8.5cm]{TZavailability2.pdf}
    \caption{ ARM TrustZone (TZ) availability in the portfolio of five top global MCU Vendors in February 2021 .
    \cite{cypressMicrocontrollerPortfolioInfineon,microchipNewPopular32bit,NuvotonM261M262,nxpProductSelectorNXP,stmicroelectronicsSTMCUFINDERPCSTM32STM8}.  }
    \label{fig:TZavailablity}

\end{figure}

We also surveyed the vendors' portfolios to identify the availability
of MPU and DMA controllers on commercial devices.  The information
related to the MPU is not listed directly in the online catalogs
published by all top vendors.  However, ST Microelectronics provides a
complete database that we used as a reference for our survey.  The
result presented in Figure \ref{fig:DmaMPUtz} demonstrates that 100\%
of the commercial Cortex-M devices have a \dctr.  A comparable result
(i.e., 94.1\%) for the Microchip portfolio was reported by
\cite{meraDICEAutomaticEmulation2021}.  In terms of MPU availability,
743 devices (i.e., 77.1\%) support this component -- including all the
latest Armv8-M devices supporting TrustZone.

\begin{figure}
    \centering
    \includegraphics[width=3cm]{dmamputz.pdf}
    \caption{ MPU and \dctr availability in the ST Microelectronics portfolio in February 2021. 
    \cite{STMCUFINDERSTM32STM8}.  }
    \label{fig:DmaMPUtz}

\end{figure}


